Adaptive-Latency DRAM (AL-DRAM)

This paper summarizes the idea of Adaptive-Latency DRAM (AL-DRAM), which was published in HPCA 2015. The key goal of AL-DRAM is to exploit the extra margin that is built into the DRAM timing parameters to reduce DRAM latency. The key observation is that the timing parameters are dictated by the worst-case temperatures and worst-case DRAM cells, both of which lead to small amount of charge storage and hence high access latency. One can therefore reduce latency by adapting the timing parameters to the current operating temperature and the current DIMM that is being accessed. Using an FPGA-based testing platform, our work first characterizes the extra margin for 115 DRAM modules from three major manufacturers. The experimental results demonstrate that it is possible to reduce four of the most critical timing parameters by a minimum/maximum of 17.3%/54.8% at 55C while maintaining reliable operation. AL-DRAM adaptively selects between multiple different timing parameters for each DRAM module based on its current operating condition. AL-DRAM does not require any changes to the DRAM chip or its interface; it only requires multiple different timing parameters to be specified and supported by the memory controller. Real system evaluations show that AL-DRAM improves the performance of memory-intensive workloads by an average of 14% without introducing any errors.

==> sec/9_relatedwork.tex <==
\section{Related Work}

Several works investigated the possibility of reducing DRAM latency by either
exploiting DRAM latency variation~\cite{Chandrasekar2014, nuat} or changing the
DRAM architecture~\cite{fcram, rldram, tldram, ahn13, salp, rowclone}. We
discuss these below.

{\bf DRAM Latency Variation:} Recently, Chandrasekar et
al.~\cite{Chandrasekar2014} evaluate the potential of relaxing some DRAM timing
parameters to reduce DRAM latency. This work observes latency variations across
DIMMs as well as for a DIMM at different operating temperatures. However, there
is no explanation as to why this phenomenon exists. In contrast, our work {\em
(i)}~identifies and analyzes the root cause of latency variation in detail,
{\em (ii)}~provides a practical mechanism that can relax timing parameters, and
{\em (iii)}~provides a real system evaluation of this new mechanism, using real
workloads, showing improved performance and preserved reliability.

Shin et al.~\cite{nuat} show that recently-refreshed rows have more charge, and
propose a mechanism (NUAT) to access the recently-refreshed rows with reduced
latency (especially, {\tt tRCD}/{\tt tRAS}). Even though some of the
observations in~\cite{nuat} are similar to ours, the approaches to leverage
them are different. AL-DRAM exploits temperature dependence in a DIMM and
process variations across DIMMs. NUAT uses the time difference between a row
refresh and an access to the row (hence its benefits are dependent on when the
row is accessed after it is refreshed). AL-DRAM provides latency benefits
regardless of access pattern and NUAT provides latency benefits regardless of
DRAM temperature. Therefore, the two techniques are complementary and can
potentially be combined for better performance. We note that {\em (i)} \ALD has
very little overhead compared to NUAT, and {\em (ii)} compared to~\cite{nuat},
our work {\em experimentally} analyzes the dependence of DRAM latency on
temperature and process variation in {\em real} DRAM chips.

{\bf Other Methods for Lower Memory Latency:} Other methods of reducing/hiding
memory latency, e.g., by employing prefetching (e.g.,~\cite{srinath07}),
memory/cache compression (e.g.,~\cite{lcp, bdi, memzip}), better memory
scheduling (e.g.,~\cite{atlas, tcm, mcp}), or better caching
(e.g.,~\cite{eaf, khan-hpca14}), are orthogonal to our approach.


==> sty/font.tex <==
\usepackage[T1]{fontenc}
\usepackage{libertine}
\renewcommand*\oldstylenums[1]{{\fontfamily{fxlj}\selectfont #1}}

